On Robustness and Generalization of ML-Based Congestion Predictors to Valid and Imperceptible Perturbations

There is substantial interest in the use of machine learning (ML)-based techniques throughout the electronic computer-aided design (CAD) flow, particularly methods based on deep learning. However, while deep learning methods have achieved state-of-the-art performance in several applications, recent work has demonstrated that neural networks are generally vulnerable to small, carefully chosen perturbations of their input (e.g. a single pixel change in an image). In this work, we investigate robustness in the context of ML-based EDA tools -- particularly for congestion prediction. As far as we are aware, we are the first to explore this concept in the context of ML-based EDA. We first describe a novel notion of imperceptibility designed specifically for VLSI layout problems defined on netlists and cell placements. Our definition of imperceptibility is characterized by a guarantee that a perturbation to a layout will not alter its global routing. We then demonstrate that state-of-the-art CNN and GNN-based congestion models exhibit brittleness to imperceptible perturbations. Namely, we show that when a small number of cells (e.g. 1%-5% of cells) have their positions shifted such that a measure of global congestion is guaranteed to remain unaffected (e.g. 1% of the design adversarially shifted by 0.001% of the layout space results in a predicted decrease in congestion of up to 90%, while no change in congestion is implied by the perturbation). In other words, the quality of a predictor can be made arbitrarily poor (i.e. can be made to predict that a design is "congestion-free") for an arbitrary input layout. Next, we describe a simple technique to train predictors that improves robustness to these perturbations. Our work indicates that CAD engineers should be cautious when integrating neural network-based mechanisms in EDA flows to ensure robust and high-quality results.

==> figures/alg.tex <==
\begin{algorithm}
\caption{training procedure}
\begin{flushleft}
\textbf{Input:} Training data $\mathcal{D}$, validation-data set $\mathcal{\hat{D}}$, max iterations $T$, learning rates $\alpha, \beta$\\
\textbf{Output:} Classifier parameters $\theta$
\end{flushleft}
\begin{algorithmic}[1]
\State $t \gets 0$
\State Initialize $\theta_0$, $\mu_0$, $w_{0} = \omega_{\mu_{0}}(\Delta)$
\For{$t\leq T$}    
    \State $(X,y) \sim \mathcal{D}$, $(\hat{X},\hat{y}) \sim \mathcal{\hat{D}}$
    
    \State $\tilde{\theta}_t $
    \State $\mu_{t+1} = \mu_t - $ 
    \Comment{compute }

    \State compute $w_{t+1} = \omega_{\mu_{t+1}}(\Delta)$
    \Comment{compute }
    \State $\theta_{t+1} = \theta_{t} - \beta\nabla_{\theta}\hat{\mathcal{L}}_{\textrm{tr}}|_{\theta_t, w_{t+1}}$
\EndFor
\State \Return $\theta_T$
\end{algorithmic}
\label{alg:training_proc}
\end{algorithm}\begin{algorithm}
\caption{training procedure}
\begin{flushleft}
\textbf{Input:} Training data $\mathcal{D}$, validation-data set $\mathcal{\hat{D}}$, max iterations $T$, learning rates $\alpha, \beta$\\
\textbf{Output:} Classifier parameters $\theta$
\end{flushleft}
\begin{algorithmic}[1]
\State $t \gets 0$
\State Initialize $\theta_0$, $\mu_0$, $w_{0} = \omega_{\mu_{0}}(\Delta)$
\For{$t\leq T$}    
    \State $(X,y) \sim \mathcal{D}$, $(\hat{X},\hat{y}) \sim \mathcal{\hat{D}}$
    
    \State $\tilde{\theta}_t $
    \State $\mu_{t+1} = \mu_t - $ 
    \Comment{compute }

    \State compute $w_{t+1} = \omega_{\mu_{t+1}}(\Delta)$
    \Comment{compute }
    \State $\theta_{t+1} = \theta_{t} - \beta\nabla_{\theta}\hat{\mathcal{L}}_{\textrm{tr}}|_{\theta_t, w_{t+1}}$
\EndFor
\State \Return $\theta_T$
\end{algorithmic}
\label{alg:training_proc}
\end{algorithm}

==> trash/trash.tex <==
In practice, cell density-based representations of chip layouts correspond to a discrete decomposition of the chip layout area in tiles or grids. A count-based \emph{density} function is a mapping from each cell to the positive integers. We define an imperceptible perturbation of a count-based density representation of a layout according to local and global constraints.

Let $X \in \mathbb{R_+}^{n\times n}$ be such a count-based density and $\delta \in \mathbb{R_+}^{n\times n}$ by a perturbation. Without loss of generality, we can vectorize both $X$ and $\delta$ such that they lie in $\mathbb{R_+}^{n^2}$ We say that $\delta$ is an \emph{imperceptible} perturbation in the context of physical design if the following holds:
%
\begin{enumerate}
    \item Global constraint: cells cannot be added or removed from the design (i.e. the number of cells remains the same after perturbation): $\sum_i \delta_i = 0$.
    \item Local constraint: the maximum number of cells that can be moved from / to an individual tile cannot exceed $\epsilon_\infty$: $||\delta||_\infty \leq \epsilon_\infty$
    \item Local constraint: a cell can only be moved a maximum of $\epsilon_g$ tiles away
    \item Global constraint: the maximum number of tiles from which cells can be moved from / to cannot exceed $\epsilon_0$: $||\delta||_0 \leq \epsilon_0$
\end{enumerate}
%
This corresponds to solving the following optimization problem:
%
\begin{equation}
\begin{aligned}
     \delta^*_{p} = \argmax_{\delta \in \mathbb{R}^{n^2}}\langle w, \delta \rangle\quad \text{s.t. } &||\delta||_0\leq \epsilon_0, \quad ||\delta||_\infty\leq \epsilon_\infty \\
     &\sum_i \delta_i = 0, \quad \delta + x \in [0,1]^{n^2}
\label{eq:decomposed_objective}
\end{aligned}
\end{equation}
%
Let $P= I -\mathbf{1}\mathbf{1}^\top$ be the projection onto the subspace orthogonal to the unit vector $\mathbf{1}$. Without loss of generality, replacing $\delta$ with $P \delta$, we may assume that $\mathbf{1}^\top \delta = \sum_i \delta_i = 0$.

\subsubsection{Projection onto the $\ell_0+\ell_\infty$-ball}
Given $x \in [0,1]^d$, we define the feasible set\textemdash the intersection of the $\ell_0$-ball of radius $\epsilon_0$, the $\ell_\infty$-ball of radius $\epsilon_\infty$ around $x$ and the set $[0,1]^d$:
\begin{equation}
\begin{aligned}
S(x) = \{&z \in \mathbb{R}^d | \:\: \sum_{i=1}^d \mathbbm{1}_{|z_i - x_i| > 0}\leq \epsilon_0, \\
&-\epsilon_\infty \leq z_i - x_i \leq \epsilon_\infty,\:\:0 \leq z_i \leq 1 \}
\end{aligned}
\end{equation}
%
%The Euclidean projection onto $S(x)$ is then given by
%$$
%\min_z ||y - z||_2^2\quad \text{s.t. } 0 \leq z_i \leq 1, \:\:
%\sum_{i=1}^d \mathbbm{1}_{|z_i - x_i| > 0}\leq k
%$$
%
First, note that intersection of the two constraints $0 \leq z_i \leq 1$ and $-\epsilon_\infty \leq z_i - x_i \leq \epsilon_\infty$ may be written %\yucheng{Should it be $\max\{0, -\epsilon_\infty + x_i\} \leq z_i \leq \min\{1, \epsilon_\infty + x_i\} $?}:
$$
\max\{0, -\epsilon_\infty + x_i\} \leq z_i \leq \min\{1, \epsilon_\infty + x_i\} 
$$
So, the feasible set may be re-written
\begin{equation}
\begin{aligned}
S(x) = \{&z \in \mathbb{R}^d | \sum_{i=1}^d \mathbbm{1}_{|z_i - x_i| > 0}\leq \epsilon_0, \\
&\max\{0, -\epsilon_\infty + x_i\} \leq z_i \leq \min\{1, \epsilon_\infty + x_i\} \}
\end{aligned}
\end{equation}
%
The Euclidean projection onto $S(x)$ is then given by
\begin{equation}
\begin{aligned}
&\min_z ||y - z||_2^2 \\
&\text{s.t. } \sum_{i=1}^d \mathbbm{1}_{|z_i - x_i| > 0}\leq \epsilon_0, \\
&\max\{0, -\epsilon + x_i\} \leq z_i \leq \min\{1, -\epsilon + x_i\}
\end{aligned}
\end{equation}
%
Ignoring the combinatorial $\ell_0$ constraint, the solution is given by $z_{i}^* = \max\{l_i, \min\{y_i, u_i\}\}$, where $l_i = \max\{0, -\epsilon + x_i\}$ and $u_i = \min\{1, -\epsilon + x_i\}$. We can then re-integrate the $\ell_0$ constraint and resolve the projection by sorting the \emph{gain} $\phi$:
$$
\phi_i = (y_i - x_i)^2 - (y_i - z_i^*)^2,\quad
z_{\pi_i} = 
\begin{cases}
z^*_{\pi_i} \quad i=1,\ldots,k \\
x_{\pi_i} \quad \text{otherwise}
\end{cases}
$$
Thus, the final solution will have $k$ entries\textemdash those with the highest gain\textemdash and that differ by no more than $1$ or $\epsilon_\infty$. 
